Robust Data-Driven Moving Horizon Estimation for Linear Discrete-Time Systems

In this paper, a robust data-driven moving horizon estimation (MHE) scheme for linear time-invariant discrete-time systems is introduced. The scheme solely relies on offline collected data without employing any system identification step. We prove practical robust exponential stability for the setting where both the online measurements and the offline collected data are corrupted by non-vanishing and bounded noise. The behavior of the novel robust data-driven MHE scheme is illustrated by means of simulation examples and compared to a standard model-based MHE scheme, where the model is identified using the same offline data as for the data-driven MHE scheme.

==> decrease_cJ.tex <==
%% decrease_cJ

\textcolor{blue}{
	\subsection{State Estimation Error Bounds}
	\label{sec:Horizon}
	As mentioned in Section~II, we here want to show that $c_J(t) > c_J(t+1) \: \: \forall t \in \mathbb{I}_{\geq 0}$ for $\rho < \frac{p_0}{p_0 + r_0} $. To this end, we consider
	%As mentioned at the end of Section \ref{sec:RGES_nom}, the state estimation error bounds improve with increasing horizon $L$ for specific choices of $\rho$. To see this, consider the constants $P_0$ and $R_0$ that both depend on $c_J$, which in turn depends on the horizon length $L$ ($t$ in (\ref{def:cJ}) is replaced by $L$, once we consider $t \geq L$). We want to show that the bounds, i.e., the value of $c_J$, decreases if the horizon length $L$ increases. To this end, we need to show that $c_J(L) > c_J(L+1)$, i.e., it must hold that
	\begin{align*}
		p_0 \rho^t + r_0 \frac{\rho - \rho^{t+1}}{1-\rho} > p_0 \rho^{t+1} + r_0 \frac{\rho - \rho^{t+2}}{1- \rho}.
	\end{align*}
	We multiply by $1-\rho$ and subtract $r_0\rho$
	\begin{align*}
		p_0 \rho^t(1- \rho) -& r_0 \rho^{t+1} >  p_0 \rho^{t+1}(1- \rho) - r_0 \rho^{t+2}.
	\end{align*}
	Dividing by $\rho^t$ yields
	\begin{align*}
		p_0(1- \rho) -& r_0 \rho >  p_0 \rho(1- \rho) - r_0 \rho^{2}.
	\end{align*}
	This inequality can be reformulated as a quadratic expression in $\rho$
	\begin{align}
		\rho^2 - \rho \frac{2p_0 + r_0}{p_0 + r_0} + \frac{p_0}{p_0 + r_0} > 0, 
	\end{align}
	which has its zeros at $\rho_1 = 1$  and $\rho_2 = \frac{p_0}{p_0 + r_0}$. Therefore, for any $\rho < \frac{p_0}{p_0 + r_0}$, it holds that $c_J(t) > c_J(t+1) \: \: \forall t \in \mathbb{I}_{\geq 0}$.}
